Blind Motion Deblurring with Pixel-Wise Kernel Estimation via Kernel Prediction Networks

In recent years, the removal of motion blur in photographs has seen impressive progress in the hands of deep learning-based methods, trained to map directly from blurry to sharp images. For this reason, approaches that explicitly use a forward degradation model received significantly less attention. However, a well-defined specification of the blur genesis, as an intermediate step, promotes the generalization and explainability of the method. Towards this goal, we propose a learning-based motion deblurring method based on dense non-uniform motion blur estimation followed by a non-blind deconvolution approach. Specifically, given a blurry image, a first network estimates the dense per-pixel motion blur kernels using a lightweight representation composed of a set of image-adaptive basis motion kernels and the corresponding mixing coefficients. Then, a second network trained jointly with the first one, unrolls a non-blind deconvolution method using the motion kernel field estimated by the first network. The model-driven aspect is further promoted by training the networks on sharp/blurry pairs synthesized according to a convolution-based, non-uniform motion blur degradation model. Qualitative and quantitative evaluation shows that the kernel prediction network produces accurate motion blur estimates, and that the deblurring pipeline leads to restorations of real blurred images that are competitive or superior to those obtained with existing end-to-end deep learning-based methods. Code and trained models are available at https://github.com/GuillermoCarbajal/J-MKPD/.

==> figure1.tex <==
  



\begin{figure}[ht]
  \centering
  \tiny
  \setlength{\tabcolsep}{0.5pt}
  \begin{tabular}{*{3}{c}}
    \scriptsize{Blurry} & \scriptsize{Ours}  & \scriptsize{GT}  \\
    \hline
    \includegraphics[trim=20 200 350 320, clip, width=0.16\textwidth]{imgs/RealBlur/Blurry/scene044_blur_06.jpg}   &
      \includegraphics[trim=20 200 350 320, clip,width=0.16\textwidth]{imgs/RealBlur/ours_L2/scene044_blur_06.jpg} &
        \includegraphics[trim=20 200 350 320, clip,width=0.16\textwidth]{imgs/RealBlur/GT/scene044_gt_06.jpg}  \\
        PSNR=29.64, CPBD=0.403 &   PSNR=28.13, CPBD=0.729    & CPBD=0.491   \\
    \includegraphics[trim=0 150 350 320, clip, width=0.16\textwidth]{imgs/RealBlur/Blurry/scene050_blur_17.jpg}   &
      \includegraphics[trim=0 150 350 320, clip,width=0.16\textwidth]{imgs/RealBlur/ours_L2/scene050_blur_17.jpg} &  
        \includegraphics[trim=0 150 350 320, clip,width=0.16\textwidth]{imgs/RealBlur/GT/scene050_gt_17.jpg}  \\
            PSNR=30.25, CPBD=0.362  & PSNR=29.0, CPBD=0.727   & CPBD=0.496   \\
    \includegraphics[trim=200 350 100 120, clip, width=0.16\textwidth]{imgs/RealBlur/Blurry/scene103_blur_04.jpg}   &
      \includegraphics[trim=200 350 100 120, clip,width=0.16\textwidth]{imgs/RealBlur/ours_L2/scene103_blur_04.jpg} &  
        \includegraphics[trim=200 350 100 120, clip,width=0.16\textwidth]{imgs/RealBlur/GT/scene103_gt_04.jpg}  \\
         PSNR=28.47, CPBD=0.285  &  PSNR=26.01, CPBD=0.612    & CPBD=0.361\\
    \includegraphics[trim=200 200 50 200, clip, width=0.16\textwidth]{imgs/RealBlur/Blurry/scene107_blur_07.jpg}   &
      \includegraphics[trim=200 200 50 200, clip,width=0.16\textwidth]{imgs/RealBlur/ours_L2/scene107_blur_07.jpg} &
        \includegraphics[trim=200 200 50 200, clip,width=0.16\textwidth]{imgs/RealBlur/GT/scene107_gt_07.jpg}   \\
        PSNR=30.08, CPBD=0.162   & PSNR=30.67, CPBD=0.470    & CPBD=0.381\\
    \includegraphics[trim=200 200 50 250, clip, width=0.16\textwidth]{imgs/RealBlur/Blurry/scene130_blur_07.jpg}   &
      \includegraphics[trim=200 200 50 250, clip,width=0.16\textwidth]{imgs/RealBlur/ours_L2/scene130_blur_07.jpg} &  
        \includegraphics[trim=200 200 50 250, clip,width=0.16\textwidth]{imgs/RealBlur/GT/scene130_gt_07.jpg} \\
         PSNR=29.20, CPBD=0.310 & PSNR=30.52, CPBD=0.707   &   CPBD=0.413  \\
    \includegraphics[trim=250 150 50 300, clip, width=0.16\textwidth]{imgs/RealBlur/Blurry/scene208_blur_03.jpg}   &
      \includegraphics[trim=250 150 50 300, clip,width=0.16\textwidth]{imgs/RealBlur/ours_L2/scene208_blur_03.jpg} & 
        \includegraphics[trim=250 150 50 300, clip,width=0.16\textwidth]{imgs/RealBlur/GT/scene208_gt_03.jpg} \\
                       PSNR=29.24, CPBD=0.290 &   PSNR=29.07, CPBD=0.692    & CPBD=0.422 \\
  \end{tabular}
  \caption{\textbf{Deblurring on real images from \cite{rim_2020_ECCV}}. Our method produces sharp results, some even sharper than \textit{ground-truth} images. As PSNR does not correlate well with the quality of the images, we also report results on blur-specific metrics that correlate better with our perception.  Best viewed in electronic format.\label{fig:figure1} }
  
\end{figure}





==> figure_Kohler.tex <==
\begin{figure*}[t!]
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{c|ccc|ccccc}
    & \multicolumn{3}{c|}{  End-to-end } & \multicolumn{5}{c}{  Model-based} \\ [.25em]
Original &   D-GAN2 \cite{kupyn2018deblurgan} & SRN \cite{tao2018scale}     & MPRNet\cite{Zamir2021MPRNet}  & Whyte\cite{whyte2010nonuniform}   & Sun\cite{sun2015learning}    & Gong\cite{gong2017motion}  & Ana-Syn\cite{kaufman2020deblurring} & Ours  \\
\includegraphics[width=0.1\textwidth]{imgs/Kohler/Blurry/Blurry1_1.jpg} &

\includegraphics[width=0.1\textwidth]{imgs/Kohler/DeblurGANv2Inception/Blurry1_1.jpg} &   
\includegraphics[width=0.1\textwidth]{imgs/Kohler/SRN/Blurry1_1.jpg}  &
\includegraphics[width=0.1\textwidth]{imgs/Kohler/MPRNet/Blurry1_1.jpg}
& 
\includegraphics[width=0.1\textwidth]{imgs/Kohler/Whyte/Blurry1_1_result_whyteMAP-krishnan.jpg}
&
\includegraphics[width=0.1\textwidth]{imgs/Kohler/Sun/Blurry1_1.jpg}
& 
\includegraphics[width=0.1\textwidth]{imgs/Kohler/Gong/Blurry1_1_deblurred.jpg} &
\includegraphics[width=0.1\textwidth]{imgs/Kohler/anasyn/Blurry1_1.jpg} &
\includegraphics[width=0.1\textwidth]{imgs/Kohler/our/Blurry1_1_NIMBUSR.jpg}
\\ 
\includegraphics[trim=150 260 125 25, clip, width=0.1\textwidth]{imgs/Kohler/Blurry/Blurry1_1.jpg} &

\includegraphics[trim=300 520 250 50, clip,width=0.1\textwidth]{imgs/Kohler/DeblurGANv2Inception/Blurry1_1.jpg} & 
\includegraphics[trim=300 520 250 50, clip,width=0.1\textwidth]{imgs/Kohler/SRN/Blurry1_1.jpg} & 
\includegraphics[trim=300 520 250 50, clip,width=0.1\textwidth]{imgs/Kohler/MPRNet/Blurry1_1.jpg} & 
\includegraphics[trim=300 520 250 50, clip,width=0.1\textwidth]{imgs/Kohler/Whyte/Blurry1_1_result_whyteMAP-krishnan.jpg}
&
\includegraphics[trim=300 520 250 50, clip,width=0.1\textwidth]{imgs/Kohler/Sun/Blurry1_1.jpg}
&
\includegraphics[trim=300 520 250 50, clip,width=0.1\textwidth]{imgs/Kohler/Gong/Blurry1_1_deblurred.jpg} &
\includegraphics[trim=300 520 250 50, clip,width=0.1\textwidth]{imgs/Kohler/anasyn/Blurry1_1.jpg} &
\includegraphics[trim=300 520 250 50,
clip,width=0.1\textwidth]{imgs/Kohler/our/Blurry1_1_NIMBUSR.jpg}
\\ 
27.58  dB & 30.88 dB &  31.51  dB  & 33.37 dB &   34.00 dB  & 27.78 dB  &  27.45 dB & 35.70 dB &  35.49 dB \\


\includegraphics[width=0.1\textwidth]{imgs/Kohler/Blurry/Blurry3_1.jpg} &

\includegraphics[width=0.1\textwidth]{imgs/Kohler/DeblurGANv2Inception/Blurry3_1.jpg} &   
\includegraphics[width=0.1\textwidth]{imgs/Kohler/SRN/Blurry3_1.jpg}  &
\includegraphics[width=0.1\textwidth]{imgs/Kohler/MPRNet/Blurry3_1.jpg} & 
\includegraphics[width=0.1\textwidth]{imgs/Kohler/Whyte/Blurry3_1_result_whyteMAP-krishnan.jpg} 
&
\includegraphics[width=0.1\textwidth]{imgs/Kohler/SRN/Blurry3_1.jpg} 
&
\includegraphics[width=0.1\textwidth]{imgs/Kohler/Gong/Blurry3_1_deblurred.jpg} &
\includegraphics[width=0.1\textwidth]{imgs/Kohler/anasyn/Blurry3_1.jpg} &
\includegraphics[width=0.1\textwidth]{imgs/Kohler/our/Blurry3_1_NIMBUSR.jpg}
\\ 
\includegraphics[trim=150 120 100 125, clip, width=0.1\textwidth]{imgs/Kohler/Blurry/Blurry3_1.jpg} &
\includegraphics[trim=300 240 200 250, clip,width=0.1\textwidth]{imgs/Kohler/DeblurGANv2Inception/Blurry3_1.jpg} &  
\includegraphics[trim=300 240 200 250, clip,width=0.1\textwidth]{imgs/Kohler/SRN/Blurry3_1.jpg}  &
\includegraphics[trim=300 240 200 250, clip,width=0.1\textwidth]{imgs/Kohler/MPRNet/Blurry3_1.jpg}  & 
\includegraphics[trim=300 240 200 250, clip,width=0.1\textwidth]{imgs/Kohler/Whyte/Blurry3_1_result_whyteMAP-krishnan.jpg}
&
\includegraphics[trim=300 240 200 250, clip,width=0.1\textwidth]{imgs/Kohler/Sun/Blurry3_1.jpg}
& 
\includegraphics[trim=300 240 200 250, clip,width=0.1\textwidth]{imgs/Kohler/Gong/Blurry3_1_deblurred.jpg} 
&
\includegraphics[trim=300 240 200 250, clip,width=0.1\textwidth]{imgs/Kohler/anasyn/Blurry3_1.jpg} &
\includegraphics[trim=300 240 200 250, clip,width=0.1\textwidth]{imgs/Kohler/our/Blurry3_1_NIMBUSR.jpg}
\\ 

27.53 dB & 31.32 dB & 32.21 dB   & 26.54 dB &  36.25 dB & 27.94 dB & 27.55 dB & 35.36 dB & 35.96 dB  \\
    \end{tabular}
    \caption{\textbf{Qualitative comparison of different deblurring methods on real images from the  K\"{o}hler Dataset~\cite{kohler2012recording}.}  %
    }
    \label{fig:kohlerDataset}
\end{figure*}


==> figure_RealBlur_DeblurGANv2_vs_JMKPD.tex <==
\begin{figure*}[ht]
  \centering
  \scriptsize
\setlength{\tabcolsep}{2pt}
  \begin{tabular}{*{4}{c}}
            Blurry & DeblurGAN-v2-Inception & J-MKPD & Ground truth \\
    \includegraphics[trim=70 195 300 270, clip, width=0.24\textwidth]{imgs/RealBlur/Blurry/scene205_blur_06.png}   &
      \includegraphics[trim=70 195 300 270, clip,width=0.24\textwidth]{imgs/RealBlur/DeblurGAN-v2-inception/scene205_blur_06.jpg}   &
      \includegraphics[trim=70 195 300 270, clip,width=0.24\textwidth]{imgs/RealBlur/COCO900_restL2_aug_all_loss_gf1_80k/restored/scene205_blur_06.jpg} &  
        \includegraphics[trim=70 195 300 270, clip,width=0.24\textwidth]{imgs/RealBlur/GT/scene205_gt_06.jpg}\\
      &   PSNR=33.11 dB/ LPIPS=0.086  & PSNR=32.41 dB/ LPIPS=0.114 & \\
    \includegraphics[trim=20 220 350 320, clip, width=0.24\textwidth]{imgs/RealBlur/Blurry/scene044_blur_06.jpg}   &
      \includegraphics[trim=20 220 350 320, clip,width=0.24\textwidth]{imgs/RealBlur/DeblurGAN-v2-inception/scene044_blur_06.jpg}   &
      \includegraphics[trim=20 220 350 320, clip,width=0.24\textwidth]{imgs/RealBlur/COCO900_restL2_aug_all_loss_gf1_80k/restored/scene044_blur_06.jpg} &  
        \includegraphics[trim=20 220 350 320, clip,width=0.24\textwidth]{imgs/RealBlur/GT/scene044_gt_06.jpg}\\
 &  PSNR=30.08 dB/ LPIPS=0.060 &  PSNR=28.13 dB/ LPIPS=0.132 & \\
    \includegraphics[trim=0 170 350 320, clip, width=0.24\textwidth]{imgs/RealBlur/Blurry/scene050_blur_17.jpg}   &
      \includegraphics[trim=0 170 350 320, clip,width=0.24\textwidth]{imgs/RealBlur/DeblurGAN-v2-inception/scene050_blur_17.jpg}   & 
    \includegraphics[trim=0 170 350 320, clip,width=0.24\textwidth]{imgs/RealBlur/COCO900_restL2_aug_all_loss_gf1_80k/restored/scene050_blur_17.jpg} &  
        \includegraphics[trim=0 170 350 320, clip,width=0.24\textwidth]{imgs/RealBlur/GT/scene050_gt_17.jpg}\\
 & PSNR=30.86 dB/ LPIPS=0.081 & PSNR=29.12 dB/ LPIPS=0.119 & \\
    \includegraphics[trim=200 350 100 120, clip, width=0.24\textwidth]{imgs/RealBlur/Blurry/scene103_blur_04.jpg}   &
      \includegraphics[trim=200 350 100 120, clip,width=0.24\textwidth]{imgs/RealBlur/DeblurGAN-v2-inception/scene103_blur_04.jpg}   &
      \includegraphics[trim=200 350 100 120, clip,width=0.24\textwidth]{imgs/RealBlur/COCO900_restL2_aug_all_loss_gf1_80k/restored/scene103_blur_04.jpg} &  
        \includegraphics[trim=200 350 100 120, clip,width=0.24\textwidth]{imgs/RealBlur/GT/scene103_gt_04.jpg}\\
         &  PSNR=28.72 dB/ LPIPS=0.068 & PSNR=26.05 dB/ LPIPS=0.128 & \\
    \includegraphics[trim=200 200 50 250, clip, width=0.24\textwidth]{imgs/RealBlur/Blurry/scene130_blur_07.jpg}   &
      \includegraphics[trim=200 200 50 250, clip,width=0.24\textwidth]{imgs/RealBlur/DeblurGAN-v2-inception/scene130_blur_07.jpg}   &
       \includegraphics[trim=200 200 50 250, clip,width=0.24\textwidth]{imgs/RealBlur/COCO900_restL2_aug_all_loss_gf1_80k/restored/scene130_blur_07.jpg} &  
        \includegraphics[trim=200 200 50 250, clip,width=0.24\textwidth]{imgs/RealBlur/GT/scene130_gt_07.jpg}\\
      & PSNR=32.38 dB/ LPIPS=0.063 & PSNR=30.45 dB/ LPIPS=0.103 & \\
    \includegraphics[trim=180 280 80 150, clip, width=0.24\textwidth]{imgs/RealBlur/Blurry/scene209_blur_09.jpg}   &
      \includegraphics[trim=180 280 80 150, clip,width=0.24\textwidth]{imgs/RealBlur/DeblurGAN-v2-inception/scene209_blur_09.jpg}   &
        \includegraphics[trim=180 280 80 150, clip,width=0.24\textwidth]{imgs/RealBlur/COCO900_restL2_aug_all_loss_gf1_80k/restored/scene209_blur_09.jpg} &  
        \includegraphics[trim=180 280 80 150, clip,width=0.24\textwidth]{imgs/RealBlur/GT/scene209_gt_09.jpg}\\
    & PSNR=30.70 dB/ LPIPS=0.104 & PSNR=30.57 dB/ LPIPS=0.117& \\
  \end{tabular}
  \caption{\textbf{Results comparison with DeblurGAN-v2 on the RealBlur dataset~\cite{rim_2020_ECCV}.} Our method produces perceptually better restorations. However, with-reference metrics such as PSNR and LPIPS favor blurry outcomes. Best viewed in electronic format. }
  \label{fig:RealBlurComparison_DeblurGAN}
\end{figure*}

==> figure_kernes_masks_Blurry2_1.tex <==
\begin{figure}[h]
    \centering
    \setlength{\tabcolsep}{0.5pt}
    \begin{tabular}{*{15}{c}}
    \multicolumn{3}{r}{  Basis element} & 7 & 9 & 5 & 1& 18 & 21 & 3 & 2 & 24 & 23 & 17 & 0 \\
     \multicolumn{3}{r}{  } & \includegraphics[width=0.06\textwidth]
    {imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_0.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_1.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_2.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_3.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_4.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_5.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_6.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_7.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_8.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_9.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_10.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_11.jpg} \\
     \multicolumn{3}{r}{  Element contribution}  & 0.239 & 0.235 & 0.204 & 0.122 & 0. 055 & 0.043 & 0.035 & 0.020 & 0.016 & 0.016 & 0.016 & 0.000 \\ 
     \multicolumn{3}{r}{} & \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_0_cumulative.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_1_cumulative.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_2_cumulative.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_3_cumulative.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_4_cumulative.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_5_cumulative.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_6_cumulative.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_7_cumulative.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_8_cumulative.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_9_cumulative.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_10_cumulative.jpg} &
    \includegraphics[width=0.06\textwidth]{imgs/kernels_masks/COCO900_restL2_sat_gf1/kernel_COCO900_restL2_sat_gf1_200_200_11_cumulative.jpg} \\
      \multicolumn{3}{l}{  Cumulative contribution} & 0.239 & 0.474 & 0.678 & 0.800 & 0.855 & 0.898 & 0.933 & 0.953 & 0.969 & 0.984 & 1.000 & 1.000 \\ 
    \end{tabular}
    \caption{Kernel formation process from the predicted set of kernel basis elements and corresponding mixing coefficients. The kernel corresponds to the one estimated for the central pixel of the blurry image in Fig. 5 of the revised manuscript. {\bf Top row:} basis elements with non-zero contribution, ordered from high to low contribution. {\em Bottom row:} cumulative contribution to the final kernel.}
    \label{fig:kernels_masks_cumulative}
\end{figure}

==> section_deep_plug_and_play_deconvolution.tex <==

Deep unfolding methods integrate model-based methods and learning-based methods.  Unfolding of specific optimization algorithms (e.g., half-quadratic splitting [2], alternating direction method of multipliers [6], and primal-dual [1, 9]) have been proposed to solve different image restoration tasks. 

\noindent {\bf ADMM Restoration}

In this work, we consider the optimization model

\begin{equation}
   \begin{array}{l}
\text{minimize    } f(\mathbf{x}) + h(\mathbf{z}) \\
\text{subject to    } \mathbf{Ax}+ \mathbf{Bz} = 0
\end{array} 
\label{eq:ADMM_optimization_problem}
\end{equation}

where $h$ is differentiable and can be non-convex. $f$ can be non-convex and non-differentiable.   

The augmented Lagrangian function  (\cite{boyd2011distributed,liu2019linearized}) is defined  as follows:

\begin{equation}
    L_{\beta}(\mathbf{x},\mathbf{z}, \mathbf{\gamma}) =  f(\mathbf{x}) + h(\mathbf{z}) + < \mathbf{\gamma}, \mathbf{Ax}+ \mathbf{Bz} > + \frac{\beta}{2} \Vert \mathbf{Ax}+ \mathbf{Bz} \Vert^2
    \label{ec:Lagrangian}
\end{equation}

where $\mathbf{\gamma}$ is the Lagrangian \textit{dual variable} and $\beta>0$ is called the \textit{penalty parameter}. The ADMM method solves this optimization problem iteratively with the following update rules:

\begin{equation}
    \begin{array}{cl}
     \mathbf{x}^{k+1} =& \arg \min_\mathbf{x}   L_{\beta}(\mathbf{x},\mathbf{z}^k, \mathbf{\gamma}^k) \\
     \mathbf{z}^{k+1} =& \arg \min_\mathbf{z}   L_{\beta}(\mathbf{x}^{k+1},\mathbf{z}, \mathbf{\gamma}^k)\\
     \mathbf{\gamma}^{k+1} =& \mathbf{\gamma}^{k} + \beta \left( \mathbf{A}\mathbf{x}^{k+1}+ \mathbf{\beta} \mathbf{z}^{k+1}\right)
\end{array}
\end{equation}

\noindent {\bf Scaled form}

ADMM can be written in a slightly different form, which is often more convenient, by combining the linear and quadratic terms in the augmented Lagrangian and scaling the dual variable 

\begin{equation}
\left\{
\begin{array}{cl}
     \mathbf{x}^{k+1} =& \arg \min_\mathbf{x}   \left( f(\mathbf{x}) + \frac{\beta}{2} \Vert \mathbf{A}\mathbf{x}  + \mathbf{B}\mathbf{z}^k + \mathbf{w}^k) \Vert^2  \right) \\
     \mathbf{z}^{k+1} =& \arg \min_\mathbf{z}   \left( h(\mathbf{z}) + \frac{\beta}{2} \Vert \mathbf{A}\mathbf{x}^{k+1}  + \mathbf{B}\mathbf{z} + \mathbf{w}^k) \Vert^2  \right) \\
     \mathbf{w}^{k+1} =& \mathbf{w}^{k} +  \mathbf{A}\mathbf{x}^{k+1}+ \mathbf{B} \mathbf{z}^{k+1}
\end{array}
\right.
\label{Eq:ADMM_scaled}
\end{equation}

where $\mathbf{w} = \frac{1}{\beta} \mathbf{\gamma}$ is the \textit{scaled dual variable} \cite{boyd2011distributed}. 

\noindent {\bf Scaled ADMM for deblurring}

In the particular case of deblurring, the maximization of the posterior density $p(\mathbf{x}|\mathbf{y})$ leads to the following optimization problem to compute the MAP estimator:

\begin{equation}
    \mathbf{x} = \arg \min \frac{1}{2\sigma^2} \Vert \mathbf{H}\mathbf{x} - \mathbf{y}\Vert^2 + \lambda \Phi(\mathbf{x})  
\end{equation}

which can be written in the Eq~\ref{eq:ADMM_optimization_problem} form, by defining the latent variable $\mathbf{z}=\mathbf{H}\mathbf{x}$

\begin{equation}
    \begin{array}{ll}
       f(\mathbf{x})= \lambda \Phi(\mathbf{x})  &  h(\mathbf{z})= \frac{1}{2\sigma^2} \Vert \mathbf{z} - \mathbf{y}  \Vert^2 \\
        \mathbf{A}= \mathbf{H}  & \mathbf{B}= -\mathbf{I} 
    \end{array}
\end{equation}

and the z-update in Eq~\ref{Eq:ADMM_scaled} has a closed-form solution \cite{laroche2022deep} 

\begin{equation}
    \mathbf{z}^* = \frac{ \mathbf{y} + \beta \sigma^2 (\mathbf{H}\mathbf{x}^{k+1} + \mathbf{w}^k)}{1+\beta\sigma^2}
    \label{Eq:z_update_closed_form}
\end{equation}

In general, it is not possible to obtain a closed-form solution for the subproblems in \ref{Eq:ADMM_scaled} and therefore   


\noindent {\bf Linearized ADMM}

In the $(k+1)th$ update of $\mathbf{x}$, we replace $\frac{\beta}{2} \Vert \mathbf{A}\mathbf{x}+ \mathbf{B}\mathbf{z}^k + \mathbf{w}^k \Vert_2^2$ by its approximation

\begin{equation}
\begin{split}
\frac{\beta}{2} \Vert \mathbf{A}\mathbf{x}^k+ \mathbf{B}\mathbf{z}^k + \mathbf{w}^k \Vert_2^2 + \\  < \mathbf{x} - \mathbf{x}^k , \beta \mathbf{A}^T \left( \mathbf{A} \mathbf{x}^k + \mathbf{B} \mathbf{z}^k + \mathbf{w}^k \right) > +  \frac{L_x}{2} \Vert \mathbf{x}- \mathbf{x}^k\Vert^2 
\end{split}
\end{equation}

which is a linearized term plus a regularization term ($L_x>~0$)

In the $(k+1)th$ update of $\mathbf{z}$, we replace $h(\mathbf{z})$ by its approximation

\begin{equation}
h(\mathbf{z}^k) + < \mathbf{z} - \mathbf{z}^k , \nabla h( \mathbf{z}) > + \frac{L_z}{2} \Vert \mathbf{z}- \mathbf{z}^k\Vert^2     
\end{equation}

which again is a linearized term plus a regularization term ($L_z>0$)

Replacing the corresponding parts in Lagrangian function with their approximations derived above, and removing constants factors we obtain

\begin{equation}
\begin{split}
    \hat{f}^k(\mathbf{x}) = f(\mathbf{x})  + < \mathbf{x} - \mathbf{x}^k , \beta \mathbf{A}^T \left( \mathbf{A} \mathbf{x}^k + \mathbf{B} \mathbf{z}^k +  \mathbf{w}^k \right) > + \\ 
    \frac{L_x}{2} \Vert \mathbf{x}- \mathbf{x}^k\Vert^2  
\end{split}
\end{equation}

\begin{equation}
\begin{split}
    \hat{h}^k(\mathbf{z}) =  < \mathbf{z} - \mathbf{z}^k ,\nabla h( \mathbf{z}^k) > + \frac{L_z}{2} \Vert \mathbf{z} - \mathbf{z}^k\Vert^2  +  \frac{\beta}{2} \Vert \mathbf{A}\mathbf{x}^{k+1} +  \\ \Vert \mathbf{B}\mathbf{z}+\mathbf{w}^k \Vert^2 
\end{split}
\end{equation}

which leads to

\begin{equation}
    \left\{ \begin{array}{cl}
    \mathbf{x}^{k+1} =& \arg \min_\mathbf{x}  \hat{f}(\mathbf{x})  \\
     \mathbf{z}^{k+1} =& \arg \min_\mathbf{z}   \hat{h}(\mathbf{z})  \\
     \mathbf{w}^{k+1} =& \mathbf{w}^{k} +  \mathbf{A}\mathbf{x}^{k+1}+ \mathbf{B} \mathbf{z}^{k+1} 
\end{array} 
\label{ec:linearizedADMM}
\right.
\end{equation}

The solution to Eq~\ref{ec:linearizedADMM} is

\begin{equation}
\scriptsize{
\left\{
    \begin{array}{cl}
     \mathbf{x}^{k+1} =& \textbf{prox}_{f/Lx} \lbrace{ \mathbf{x}^k - \tilde{\mathbf{x}}^k \rbrace}\\
     \mathbf{z}^{k+1} =&  (L_z + \beta \mathbf{B}^T\mathbf{B})^{-1} \left( L_z \mathbf{z}^k - \nabla h (\mathbf{z}^k)  - \beta \mathbf{B}^T ( \mathbf{A} \mathbf{x}^{k+1} +  \mathbf{w}^{k}) \right) \\
     \mathbf{w}^{k+1} =& \mathbf{w}^{k} +  \mathbf{A}\mathbf{x}^{k+1}+ \mathbf{B} \mathbf{z}^{k+1} 
\end{array}\right.
}
\end{equation}


where $\textbf{prox}_{f/Lx}$ is the \textit{proximal operator} of $f/Lx$, and

$$
\tilde{\mathbf{x}}^k = \frac{\beta}{L_x}  \mathbf{A}^T \left( \mathbf{A}\mathbf{x}^{k}+ \mathbf{B} \mathbf{z}^{k} + \mathbf{w}^{k} \right)
$$


\noindent {\bf Linearized ADMM for deblurring}

Therefore:

\begin{equation}
\left\{
\begin{array}{cl}
     \mathbf{x}^{k+1} =& \textbf{prox}_{f/Lx} \lbrace{ \mathbf{x}^k - \tilde{\mathbf{x}}^k \rbrace}\\
     \mathbf{z}^{k+1} =&  \frac{1}{L_z + \beta} \left( L_z \mathbf{z}^k - \nabla h (\mathbf{z}^k) + \beta ( \mathbf{H}  \mathbf{x}^{k+1} + \mathbf{w}^k  )\right) \\
     \mathbf{w}^{k+1} =& \mathbf{w}^{k} +  \mathbf{A}\mathbf{x}^{k+1}+ \mathbf{B} \mathbf{z}^{k+1} 
\end{array} \right.
\label{eq:linADMM_sol}
\end{equation}

Noting that $\nabla h = \frac{1}{\sigma^2}(\mathbf{z}-\mathbf{y})$ and replacing en Eq~\ref{eq:linADMM_sol} we get the following z-update for linearized ADMM:

\begin{equation}
\scriptsize{
\begin{array}{cl}
 \mathbf{z}^{k+1}  & =  \frac{1}{L_z + \beta} \left( L_z \mathbf{z}^k - \frac{1}{\sigma^2} (\mathbf{z}^k-\mathbf{y})  +  \beta ( \mathbf{H} \mathbf{x}^{k+1} +  \mathbf{w}^{k})  \right) \\
 & =   \frac{1}{(L_z + \beta) \sigma^2} \left( (\sigma^2 L_z -1)\mathbf{z}^k  + \mathbf{y}   + \sigma^2 \beta  ( \mathbf{H} \mathbf{x}^{k+1}+\mathbf{w}^{k}) \right)
 \end{array}
 }
\end{equation}

\noindent {\bf Deblurring with saturated pixels}

Considering the saturation function $R(\mathbf{z})$, the data term $h(\mathbf{z})$ becomes 

\begin{equation}
h_{sat}(\mathbf{z}) = \frac{1}{2\sigma^2} \Vert R(\mathbf{z}) - \mathbf{y} \Vert^2     
\end{equation}

and its linearization around $\mathbf{z}^k$

\begin{equation}
\scriptsize{
\hat{h}_{sat}(\mathbf{z}) =h_{sat}(\mathbf{z}^k) +  <\mathbf{z}-\mathbf{z_k}, \frac{ 1}{\sigma^2} (R(\mathbf{z_k})-\mathbf{y})R'(\mathbf{z_k})> + \frac{L_z}{2}\Vert \mathbf{z}-\mathbf{z_k}  \Vert^2 
}
\end{equation}


Therefore, the cost (linearized) to be minimized is

\begin{equation}
\scriptsize{
\hat{F}(\mathbf{z}) = <\mathbf{z}-\mathbf{z_k}, \frac{(R(\mathbf{z_k})-\mathbf{y})R'(\mathbf{z_k})}{\sigma^2}>  + \frac{L_z}{2}\Vert \mathbf{z}-\mathbf{z_k}  \Vert^2 + \frac{\beta}{2} \Vert \mathbf{z} -  (\mathbf{H}\mathbf{x}^{k+1} + \mathbf{w}^k)) \Vert^2 
}
\end{equation}

Again, we want $\nabla \hat{F}(\mathbf{z})  = 0$

\begin{equation}
\scriptsize{
\begin{array}{cl}
     \nabla  \hat{F}(\mathbf{z}) & = \frac{1}{\sigma^2}(R(\mathbf{z}^k)-\mathbf{y})R'(\mathbf{z}^k) + L_z ( \mathbf{z}-\mathbf{z}^k) + \beta ( \mathbf{z}- (\mathbf{H}\mathbf{x}^{k+1} + \mathbf{w}^k) )\\
     & = (L_z + \beta) \mathbf{z} + \frac{1}{\sigma^2}(R(\mathbf{z}^k)-\mathbf{y})R'(\mathbf{z}^k) - L_z \mathbf{z}^k -\beta (\mathbf{H}\mathbf{x}^{k+1} + \mathbf{w}^k ) \\
     &= 0 
\end{array}
}
\end{equation}

Finally, 

\begin{equation}
\scriptsize{
\begin{array}{cl}
     \mathbf{z} & = \frac{1}{(L_z + \beta)\sigma^2} \left( \left(\mathbf{y} - R(\mathbf{z}^k) \right) R'(\mathbf{z}^k) + \sigma^2 L_z  \mathbf{z}^k + \beta \sigma^2 (\mathbf{H}\mathbf{x}^{k+1} + \gamma^k ) \right) 
\end{array}
\label{eq:LinADMM_saturated}
}
\end{equation}



==> section_deep_plug_and_play_short.tex <==
In a variational approach, the deblurring problem taking into account saturation is given by 
\begin{equation}
    \mathbf{x} = \arg \min \frac{1}{2\sigma^2} \Vert R(\mathbf{H}\mathbf{x}) - \mathbf{y}\Vert^2 + \lambda \Phi(\mathbf{x}),  
\end{equation}
where $\mathbf{x}$ denotes the latent sharp image, $\mathbf{y}$ the observed blurry image, $\mathbf{H}$ the degradation matrix, $R(\cdot)$ the \textit{saturation response function}, and $\Phi(\mathbf{x})$ the \textit{prior} associated with $\mathbf{x}$.

This problem can be written in the form:

\begin{equation}
   \begin{array}{l}
\text{minimize    } f(\mathbf{x}) + h(\mathbf{z}) \\
\text{subject to    } \mathbf{Ax}+ \mathbf{Bz} = 0
\end{array} 
\label{eq:ADMM_optimization_problem}
\end{equation}

with 

\begin{equation}
    \begin{array}{ll}
       f(\mathbf{x})= \lambda \Phi(\mathbf{x})  &  h(\mathbf{z})= \frac{1}{2\sigma^2} \Vert R(\mathbf{z}) - \mathbf{y}  \Vert^2 \\
        \mathbf{A}= \mathbf{H}  & \mathbf{B}= -\mathbf{I} 
    \end{array}
\end{equation}

This leads to the alternate solution

\begin{equation}
\left\{
\begin{array}{cl}
     \mathbf{x}^{k+1} =& \arg \min_\mathbf{x}   \left( f(\mathbf{x}) + \frac{\beta}{2} \Vert \mathbf{H}\mathbf{x}  -\mathbf{z}^k + \mathbf{w}^k) \Vert^2  \right) \\
     \mathbf{z}^{k+1} =& \arg \min_\mathbf{z}   \left( h(\mathbf{z}) + \frac{\beta}{2} \Vert \mathbf{H}\mathbf{x}^{k+1}  - \mathbf{z} + \mathbf{w}^k) \Vert^2  \right) \\
     \mathbf{w}^{k+1} =& \mathbf{w}^{k} +  \mathbf{H}\mathbf{x}^{k+1} - \mathbf{z}^{k+1}
\end{array}
\right.
\label{Eq:ADMM_scaled}
\end{equation}

where $\mathbf{w} = \frac{1}{\beta} \mathbf{\gamma}$ is the \textit{scaled dual variable} \cite{boyd2011distributed}. 

As in~\cite{laroche2022deep}, \cref{Eq:ADMM_scaled} is solved using the linearized version of  the Alternating Direction Method of Multipliers (ADMM). Linearizing $\frac{\beta}{2} \Vert \mathbf{A}\mathbf{x}+ \mathbf{B}\mathbf{z}^k + \mathbf{w}^k \Vert_2^2$ in the $\mathbf{x}$-update and $h(\mathbf{z})$ in the $\mathbf{z}$-update,  the solution to \cref{Eq:ADMM_scaled} becomes

\begin{equation}
\scriptsize{
\left\{
    \begin{array}{cl}
     \mathbf{x}^{k+1} =& \textbf{prox}_{f/Lx} \lbrace{ \mathbf{x}^k - \tilde{\mathbf{x}}^k \rbrace}\\
     \mathbf{z}^{k+1} =& \frac{1}{(L_z + \beta)\sigma^2} \left( \left(\mathbf{y} - R(\mathbf{z}^k) \right) R'(\mathbf{z}^k) + \sigma^2 L_z  \mathbf{z}^k + \beta \sigma^2 (\mathbf{H}\mathbf{x}^{k+1} + \gamma^k ) \right)  \\ 
     \mathbf{w}^{k+1} =& \mathbf{w}^{k} +  \mathbf{A}\mathbf{x}^{k+1}+ \mathbf{B} \mathbf{z}^{k+1} 
\end{array}\right.
}
\end{equation}


where $\textbf{prox}_{f/Lx}$ is the \textit{proximal operator} of $f/Lx$, $L_x$ and $L_z$ are regularization factors, and

$$
\tilde{\mathbf{x}}^k = \frac{\beta}{L_x}  \mathbf{H}^T \left( \mathbf{H}\mathbf{x}^{k} - \mathbf{z}^{k} + \mathbf{w}^{k} \right)
$$

==> supp_mat_kernels_masks.tex <==
\section{Learning of Kernel Prediction Network}

Given a blurry image, the \textit{Kernel Prediction Network} predicts a basis of kernels and the corresponding mixing coefficients. The number of (kernels, mixing coefficients) pairs that can generate the estimated kernel is infinite. Since we are not interested in any particular pair, we just let the network learn how to predict the pair without any constraint. 

Previous motion estimation methods \cite{gong2017motion, zhang2021exposure} learn how to predict motion vectors by minimizing a re-blur loss. Since the estimation is local, and in many regions of the image there is not enough information to uniquely infer the motion vector, the motion map must be regularized. In contrast to those articles, we did not have to constrain the kernel basis nor the mixing coefficients to obtain smooths kernel maps. The reason that explains this behavior is that during training, we used a \textit{kernel loss} in addition to the \textit{reblur loss}.  

In \cref{fig:kernels_grid_different_losses}, we show the kernels estimated for crops in the GoPro dataset. The first columns show the kernels estimated when there is no \textit{kernel loss} during training. The kernels obtained are dotted. This may be by the combination of two factors: a) during training, there is not enough information to learn clearly delimited kernels b) the kernels in the GoPro dataset are \textit{dotted} due to blurry images generated by averaging consecutive frames. Adding the \textit{kernel loss} acts as a prior that contributes to generating continuous, well-shaped kernels. \cite{zhang2021exposure} compare different estimation methods using the reblur performance on the GoPro dataset. In \cref{tab:reblur_performance_NoFC}, we show the reblur performance for the methods trained with: a) \textit{reblur loss} on the GoPro dataset, b) kernels and reblur loss on the GoPro dataset and a synthetic dataset c) kernels and reblur loss only using the synthetic dataset. The reblur performance is much better when using the reblur loss on the GoPro dataset. However, the quality of the kernels improves considerably when adding the \textit{kernels loss}.  In \cref{fig:kernels_grid_Kohler} and  \cref{fig:kernels_grid_Lai}, we show the kernels map obtained on real images from the K\"{o}hler and the Lai dataset. Again, the kernels' better quality when using the \textit{kernels loss} is observed. 

\begin{figure}
    \centering
    \begin{tabular}{*{3}{c}} 
    (a) & (b) & (c) \\
    \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_GoPro_only_reblur_gc/0249_kernels_grid.jpg} &
    \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_ADE_GoPro_aug_gc_from_scratch/0249_kernels_grid.jpg}  &   
 \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks/first_round/0249_kernels_grid.jpg}   \\
 \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_GoPro_only_reblur_gc/0316_kernels_grid.jpg} &
    \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_ADE_GoPro_aug_gc_from_scratch/0316_kernels_grid.jpg}  &   
 \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks/first_round/0316_kernels_grid.jpg}   
    \end{tabular}
    \caption{Caption}
    \label{fig:kernels_grid_different_losses}
\end{figure}

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
         Training Set &  Loss  &  PSNR \\
         COCO         & Reblur + Kernels & 33.63 \\
         \hline
         GoPro &   Reblur & 38.64   \\
         GoPro + ADE &   Reblur + Kernels &  34.94  \\
         ADE &   Reblur  &    \\
         ADE &   Reblur + Kernels &    \\
    \end{tabular}
    \caption{Reblur performance with NoFC architecture}
    \label{tab:reblur_performance_NoFC}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
         Training Set &  Loss  &  PSNR \\
         GoPro &   Reblur &    \\
         GoPro + ADE &   Reblur + Kernels &  37.0  \\
         ADE &   Reblur  & 37.57   \\
         ADE &   Kernels  &  32.81  \\
         ADE &   Reblur + Kernels &    \\
    \end{tabular}
    \caption{Reblur performance with Xia architecture}
    \label{tab:reblur_performance_Xia}
\end{table}


\begin{figure}
    \centering
    \begin{tabular}{*{3}{c}} 
    (a) & (b) & (c) \\
    \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_GoPro_only_reblur_gc/butchershop.jpg} &
    \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_ADE_GoPro_aug_gc_from_scratch/butchershop.jpg}  &  
 \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks/first_round/butchershop.jpg}   \\
 \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_GoPro_only_reblur_gc/coke.jpg} &
    \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_ADE_GoPro_aug_gc_from_scratch/coke.jpg}  &   
 \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks/first_round/coke.jpg} \\
  \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_GoPro_only_reblur_gc/dinner.jpg} &
    \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_ADE_GoPro_aug_gc_from_scratch/dinner.jpg}  &   
 \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks/first_round/dinner.jpg} \\
    \end{tabular}
    \caption{Caption}
    \label{fig:kernels_grid_Lai}
\end{figure}


\begin{figure}
    \centering
    \begin{tabular}{*{3}{c}} 
    (a) & (b) & (c) \\
    \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_GoPro_only_reblur_gc/Blurry1_6.jpg} &
    \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_ADE_GoPro_aug_gc_from_scratch/Blurry1_6.jpg}  &   
 \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_GoPro_only_reblur_gc/Blurry1_6.jpg}   \\
 \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_GoPro_only_reblur_gc/Blurry2_1.jpg} &
    \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks_NoFC_ADE_GoPro_aug_gc_from_scratch/Blurry2_1.jpg}  &   
 \includegraphics[trim= 0 0 0 0, clip,width=0.33\textwidth]{imgs/kernels_masks/first_round/Blurry2_1.jpg} \\
    \end{tabular}
    \caption{Caption}
    \label{fig:kernels_grid_Kohler}
\end{figure}

\subsection{Training using only a reblur loss}

From \cref{tab:reblur_performance_NoFC} it is evident that adding the kernel loss significantly reduce the \textit{reblurring} performance on the GoPro dataset.  In addition, using only the \textit{reblur} loss trains faster. We explored the possibility of obtaining better kernels by constraining the kernel's basis and mixing coefficients predicted by the Kernel Prediction Network. L2 and Total Variation (TV) regularization was evaluated in the final kernels and also TV regularization in the base masks. Table \ref{tab:Xia_gopro_dataset_psnr_reblur} shows the reblur PSNR obtained with and without regularization and Figures  \ref{fig:kernels_grid_035_regs}  and \ref{fig:kernels_grid_276_regs} show some examples. Visually, regularized kernels are preferred, but reblur PSNR is significantly lower. Although regularizing the kernels and mask is an interesting approach to explore, we obtained a better generalization performance when adding the \textit{kernel loss} during training. Also, we found the regularized results very sensitive to the regularization parameters. It is very easy to over-regularize the solution, considerably limiting the expressivity of the Kernel Prediction Network. 

\begin{table}[ht]
    \centering
    \begin{tabular}{l|c}
         Model &         PSNR reblur   \\
         \hline
         No regularization &  40.92 \\
         Masks regularization (TV 1e-9 ) & 40.83 \\
         Masks (TV 1e-9) and kernels (L2 0.1) regularization & 40.96 \\
         Kernels regularization (L2 0.1) &  40.83 \\
         Masks regularization (TV 1e-7 ) & 39.21  \\
         Masks (TV 1e-7) and kernels (L2 1) regularization  &  37.54 \\ 
         \hline
    \end{tabular}
    \caption{Models trained from scratch for 750 epochs.}
    \label{tab:Xia_gopro_dataset_psnr_reblur}
\end{table}

\begin{figure}
     \centering
    \begin{subfigure}[t]{0.3\textwidth}
         \includegraphics[width=\textwidth]{imgs/kernels_grid/kernels_reg_01_masks_reg_1e-9/035/loss_0.0000478_psnr_43.21_img_399_blur_gt}
         \subcaption{Blurry image }
     \end{subfigure}
     \hfill
    \begin{subfigure}[t]{0.3\textwidth}
         \includegraphics[width=\textwidth]{imgs/kernels_grid/no_reg/035/loss_0.0000548_psnr_42.61_img_399_kernel_grid_estimated.jpg}
         \subcaption{No regularization. PSNR~reblur~=~42.61. }
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \includegraphics[width=\textwidth]{imgs/kernels_grid/kernels_reg_01_masks_reg_1e-9/035/loss_0.0000478_psnr_43.21_img_399_kernel_grid_estimated.jpg}
         \subcaption{Kernels regularization (L2 0.1). PSNR~reblur~=~43.21. }
     \end{subfigure}    
    \begin{subfigure}[t]{0.3\textwidth}
         \includegraphics[width=\textwidth]{imgs/kernels_grid/kernels_reg_01_masks_reg_1e-9/035/loss_0.0000478_psnr_43.21_img_399_kernel_grid_estimated.jpg}
         \subcaption{Kernels (L2 0.1) and masks (TV 1e-9). PSNR~reblur~=~43.21.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \includegraphics[width=\textwidth]{imgs/kernels_grid/masks_regularization_1e-7/035/loss_0.0000769_psnr_41.14_img_399_kernel_grid_estimated.jpg}
         \subcaption{Masks (TV 1e-7). PSNR~reblur~=~41.14.}
     \end{subfigure}
      \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \includegraphics[width=\textwidth]{imgs/kernels_grid/kernels_reg_1_masks_reg_1e-7/035/loss_0.0001029_psnr_39.88_img_399_kernel_grid_estimated.jpg}
         \subcaption{Kernels (L2 1) and masks (TV 1e-7). PSNR~reblur~=~39.88.}
     \end{subfigure}
     \caption{Training using only GoPro for \textcolor{red}{ADD} number of epochs.}
     \label{fig:kernels_grid_035_regs}
\end{figure}

\begin{figure}
     \centering
    \begin{subfigure}[t]{0.3\textwidth}
         \includegraphics[width=\textwidth]{imgs/kernels_grid/single_image/276/276_kernels_grid.jpg}
         \subcaption{Single image overfitting. PSNR~reblur = 45.63 }
     \end{subfigure}
     \hfill
    \begin{subfigure}[t]{0.3\textwidth}
         \includegraphics[width=\textwidth]{imgs/kernels_grid/no_reg/276/loss_0.0001291_psnr_38.89_img_276_kernel_grid_estimated.jpg}
         \subcaption{No regularization. PSNR~reblur~=~38.89. }
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \includegraphics[width=\textwidth]{imgs/kernels_grid/kernels_reg_01_masks_reg_1e-9/276/loss_0.0001515_psnr_38.20_img_276_kernel_grid_estimated.jpg}
         \subcaption{Kernels regularization (L2 0.1). PSNR~reblur~=~38.20. }
     \end{subfigure}    
    \begin{subfigure}[t]{0.3\textwidth}
         \includegraphics[width=\textwidth]{imgs/kernels_grid/kernels_reg_01_masks_reg_1e-9/276/loss_0.0001515_psnr_38.20_img_276_kernel_grid_estimated.jpg}
         \subcaption{Kernels (L2 0.1) and masks (TV 1e-9). PSNR~reblur~=~38.20.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \includegraphics[width=\textwidth]{imgs/kernels_grid/masks_regularization_1e-7/276/loss_0.0001389_psnr_38.57_img_276_kernel_grid_estimated.jpg}
         \subcaption{Masks (TV 1e-7). PSNR~reblur~=~38.57.}
     \end{subfigure}
      \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \includegraphics[width=\textwidth]{imgs/kernels_grid/kernels_reg_1_masks_reg_1e-7/276/loss_0.0002658_psnr_35.75_img_276_kernel_grid_estimated.jpg}
         \subcaption{Kernels (L2 1) and masks (TV 1e-7). PSNR~reblur~=~35.75.}
     \end{subfigure}
     \caption{TTraining using only GoPro for \textcolor{red}{ADD} number of epochs.}
     \label{fig:kernels_grid_276_regs}
\end{figure}


==> supp_mat_on_losses_effect.tex <==
\begin{table}[h]
    \small 
    \caption{\textbf{Cross-dataset evaluation on the RealBlurDataset \cite{rim_2020_ECCV}.} The PSNR/SSIM scores for the classical variational methods (first three rows) were taken from the RealBlur benchmark \cite{rim_2020_ECCV}. For DL-based methods, the values were computed using the models provided by the authors.
    }
    \label{tab:losses_effect_RealBlurDataset}
     \centering
    \begin{tabular}{lcccccc}
    \toprule
    Method & PSNR & SSIM & LPIPS & BS(11)$\uparrow$ & CPBD $\uparrow$ & SI $\uparrow$\\
    \midrule
\textcolor{magenta}{JMKPD (180k)} & 28.68 &  \colorbox{yellow}{0.879} & 0.148 & 0.378 & 0.427 & 3346 \\
\hdashline
\textcolor{magenta}{JMKPD (blurred)} & \colorbox{cyan}{29.04} &  \colorbox{cyan}{0.883}  & 0.146 & 0.399 & 0.336 & 2219  \\
    \bottomrule
    \end{tabular}
\end{table}
